Isotopic piecewise affine approximation of algebraic or $C^1$ varieties

We propose a novel sufficient condition establishing that a piecewise affine variety has the same topology as a variety of the sphere $\mathbb{S}^n$ defined by positively homogeneous $C^1$ functions. This covers the case of $C^1$ varieties in the projective space $\mathbb{P}^n$. We prove that this condition is sufficient in the case of codimension one and arbitrary dimension. We describe an implementation working for homogeneous polynomials in arbitrary dimension and codimension and give experimental evidences that our condition might still be sufficient in codimension greater than one.

==> install <==
#!/bin/sh

# This script installs the Nix package manager on your system by
# downloading a binary distribution and running its installer script
# (which in turn creates and populates /nix).

{ # Prevent execution if this script was only partially downloaded
oops() {
    echo "$0:" "$@" >&2
    exit 1
}

umask 0022

tmpDir="$(mktemp -d -t nix-binary-tarball-unpack.XXXXXXXXXX || \
          oops "Can't create temporary directory for downloading the Nix binary tarball")"
cleanup() {
    rm -rf "$tmpDir"
}
trap cleanup EXIT INT QUIT TERM

require_util() {
    command -v "$1" > /dev/null 2>&1 ||
        oops "you do not have '$1' installed, which I need to $2"
}

case "$(uname -s).$(uname -m)" in
    Linux.x86_64)
        hash=afa6bf82bacb18ec0d6a1fd992b718192f895023d6cea8b94b2fb35fce352ff5
        path=1sh0llzrvkah17hypza89fcd5bmm35cl/nix-2.13.3-x86_64-linux.tar.xz
        system=x86_64-linux
        ;;
    Linux.i?86)
        hash=579a79a155c93c07f23e58de1dfa766d905239315b6b8c116e0ad7ffb7b14135
        path=bg4vn61787q0l6wny81laa7al4sw5hda/nix-2.13.3-i686-linux.tar.xz
        system=i686-linux
        ;;
    Linux.aarch64)
        hash=dfbbaa86404c3efe74d87c8d4c39081affc673c8b5f64cfefc4ab0eaf84ed39b
        path=zdq06xpx6a4a1hkaqcvjj9lbd7vqd9c3/nix-2.13.3-aarch64-linux.tar.xz
        system=aarch64-linux
        ;;
    Linux.armv6l)
        hash=debcb8a09744e83fca06efc6c5eee3f6066653da27dda8e0fb861e565b93f5f5
        path=60gh3w8ikkhf547d3scyhsn7xlpp1k01/nix-2.13.3-armv6l-linux.tar.xz
        system=armv6l-linux
        ;;
    Linux.armv7l)
        hash=07a1e718e9ebfd11b0c8ba947029b5dc50a81f4e6f8ac5b8b8e3572e1ce436cb
        path=cr6g8xc66yc02avw3ih4h96dbamqc3xw/nix-2.13.3-armv7l-linux.tar.xz
        system=armv7l-linux
        ;;
    Darwin.x86_64)
        hash=2b036faeccdce4b6ba9ca4aa7971b49d13a1ee4ac13ea834fb24c4d0d7e8536a
        path=s8yj3dnxmkk8ggzzymxwm1qb3s5hk133/nix-2.13.3-x86_64-darwin.tar.xz
        system=x86_64-darwin
        ;;
    Darwin.arm64|Darwin.aarch64)
        hash=200e777b541ddbadafdbe3817dba504754fa8fb0c9d1dd3f33dee6578045ab39
        path=nh14dgrnxgd9dgg14bvbmi33dd5ipnml/nix-2.13.3-aarch64-darwin.tar.xz
        system=aarch64-darwin
        ;;
    *) oops "sorry, there is no binary distribution of Nix for your platform";;
esac

# Use this command-line option to fetch the tarballs using nar-serve or Cachix
if [ "${1:-}" = "--tarball-url-prefix" ]; then
    if [ -z "${2:-}" ]; then
        oops "missing argument for --tarball-url-prefix"
    fi
    url=${2}/${path}
    shift 2
else
    url=https://releases.nixos.org/nix/nix-2.13.3/nix-2.13.3-$system.tar.xz
fi

tarball=$tmpDir/nix-2.13.3-$system.tar.xz

require_util tar "unpack the binary tarball"
if [ "$(uname -s)" != "Darwin" ]; then
    require_util xz "unpack the binary tarball"
fi

if command -v curl > /dev/null 2>&1; then
    fetch() { curl --fail -L "$1" -o "$2"; }
elif command -v wget > /dev/null 2>&1; then
    fetch() { wget "$1" -O "$2"; }
else
    oops "you don't have wget or curl installed, which I need to download the binary tarball"
fi

echo "downloading Nix 2.13.3 binary tarball for $system from '$url' to '$tmpDir'..."
fetch "$url" "$tarball" || oops "failed to download '$url'"

if command -v sha256sum > /dev/null 2>&1; then
    hash2="$(sha256sum -b "$tarball" | cut -c1-64)"
elif command -v shasum > /dev/null 2>&1; then
    hash2="$(shasum -a 256 -b "$tarball" | cut -c1-64)"
elif command -v openssl > /dev/null 2>&1; then
    hash2="$(openssl dgst -r -sha256 "$tarball" | cut -c1-64)"
else
    oops "cannot verify the SHA-256 hash of '$url'; you need one of 'shasum', 'sha256sum', or 'openssl'"
fi

if [ "$hash" != "$hash2" ]; then
    oops "SHA-256 hash mismatch in '$url'; expected $hash, got $hash2"
fi

unpack=$tmpDir/unpack
mkdir -p "$unpack"
tar -xJf "$tarball" -C "$unpack" || oops "failed to unpack '$url'"

script=$(echo "$unpack"/*/install)

[ -e "$script" ] || oops "installation script is missing from the binary tarball!"
export INVOKED_FROM_INSTALL_IN=1
"$script" "$@"

} # End of wrapping

